Bayesian Nonparametric Kernel-Learning

Kernel methods are ubiquitous tools in machine learning. However, there is often little reason for the common practice of selecting a kernel a priori. Even if a universal approximating kernel is selected, the quality of the finite sample estimator may be greatly affected by the choice of kernel. Furthermore, when directly applying kernel methods, one typically needs to compute a $N \times N$ Gram matrix of pairwise kernel evaluations to work with a dataset of $N$ instances. The computation of this Gram matrix precludes the direct application of kernel methods on large datasets, and makes kernel learning especially difficult. In this paper we introduce Bayesian nonparmetric kernel-learning (BaNK), a generic, data-driven framework for scalable learning of kernels. BaNK places a nonparametric prior on the spectral distribution of random frequencies allowing it to both learn kernels and scale to large datasets. We show that this framework can be used for large scale regression and classification tasks. Furthermore, we show that BaNK outperforms several other scalable approaches for kernel learning on a variety of real world datasets.

==> misc.tex <==
% Crap that I don't want in the paper, but I don't want to discard yet

We consider \textit{Mercel Kernels}, which are real-valued functions $K(x,y)$ that are positive definite and symmetric over some domain $x,y\in \calX$. That is, for any function $f$ we have that:
\begin{align*}
\int \int K(x,y) f(x) f(y) \ud x\, \ud y \ge 0.
\end{align*}
Let $K_x$ be the function that is obtained by fixing the first kernel arguement at $x$, that is: $K_x(\cdot) \equiv K(x,\cdot)$. One takes the innerproduct $\idot{K_x}{K_y}_K \equiv K(x,y)$. Furthermore, one may obtain functions via linear combinations: $g(x) = \sum_{i=1}^m \alpha_i K_{x_i}(x)$. The RKHS induced by the kernel $K$ is the completion of the span of such functions; i.e. the RKHS, $\calH_K$, of $K$ is the completion of $\calH_0$ w.r.t. $\norm{\cdot}_K$ where
\begin{align*}
\calH_0 \equiv \left\{ g(x) = \sum_{i=1}^m \alpha_i K_{x_i}(x)\ : \ m \in \N^+,\ x_i\in\calX \right\}.
\end{align*}
Roughly speaking, the representor theorem states that if one is minizing a loss w.r.t. $f \in \calH_K$, that depends on the value of $f$ over input instances $\{x_i\}_{i=1}^N$: $\{f(x_i)\}_{i=1}^N$, and a regularizer $g(\norm{f}_K)$, then $f$ can be written as:
\begin{align*}
f(x) = \sum_{i=1}^N \alpha_i K_{x_i}(x),
\end{align*}
where $\alpha_i \in \R $. Thus, when optimizing over such $f$ one needs to only work of a gram matrix $\mathbf{K}\in \R^{N \times N}$, where $\mathbf{K}_{ij} = K(x_i,x_j)$. While the representor theroem simplifies the the task of optimizing over the RKHS, the computation and manipulation of the $N\times N$ Gram matrix will be prohibitive for working with big data when $N$ is in the many thousands or more.
